Test Generation Strategies for Building Failure Models and Explaining Spurious Failures

Test inputs fail not only when the system under test is faulty but also when the inputs are invalid or unrealistic. Failures resulting from invalid or unrealistic test inputs are spurious. Avoiding spurious failures improves the effectiveness of testing in exercising the main functions of a system, particularly for compute-intensive (CI) systems where a single test execution takes significant time. In this paper, we propose to build failure models for inferring interpretable rules on test inputs that cause spurious failures. We examine two alternative strategies for building failure models: (1) machine learning (ML)-guided test generation and (2) surrogate-assisted test generation. ML-guided test generation infers boundary regions that separate passing and failing test inputs and samples test inputs from those regions. Surrogate-assisted test generation relies on surrogate models to predict labels for test inputs instead of exercising all the inputs. We propose a novel surrogate-assisted algorithm that uses multiple surrogate models simultaneously, and dynamically selects the prediction from the most accurate model. We empirically evaluate the accuracy of failure models inferred based on surrogate-assisted and ML-guided test generation algorithms. Using case studies from the domains of cyber-physical systems and networks, we show that our proposed surrogate-assisted approach generates failure models with an average accuracy of 83%, significantly outperforming ML-guided test generation and two baselines. Further, our approach learns failure-inducing rules that identify genuine spurious failures as validated against domain knowledge.

==> Sections/answerMajorReview.tex <==
%%%%
%%% COMMAND USAGE:
%%% REPORTING THE COMMENT
%%% \rwcomment{commentid}{comment textual description}
%%% commentid -> an id of your choice associated with the comment
%%% comment textual descriptionn -> the original comment of the reviewer

%%% ANSWERING A COMMENT
%%% \response{The response for the question. If you want to reference some text use \referenceaddressed{idAssociated with the answer in the text of the paper}}

%%% CHANGING THE PAPER CONTENT
%% \change{new text that will be added}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}
%% \delete{text to be deleted}}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}
%% \rep{new text}{old text}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}

\noindent\textbf{Associate Editor}
\vspace*{.5cm}
\rwcomment{ARC1}{There are however some concerns from one of the reviewers regarding the novelty and existing work in the area. In addition the reviewers are asking about some clarity around the approach. These comments, while not major, they may require some time to address.}
\response{Thank you for your comment. In response to Reviewer \#2's comments, we clarify that our paper reports completely new research results and  contributions that have not been  reported in any previous work. Our paper does \emph{not} extend any existing conference or workshop paper. Therefore, our paper satisfies the conditions of the journal first category. \\
Regarding the relationship to prior work~\cite{ben2016testing,haq2022efficient}, 
we have now clarified on~\referenceaddressed{R2C4l} that these earlier papers pursue different goals and use different algorithms compared to this current manuscript. Specifically,  these earlier papers employ machine learning to more effectively steer test generation towards areas within the search space that are likely to contain the most severe failures. In this current work, we use machine learning to devise new test generation algorithms, with the aim of inferring failure models for systems with numeric inputs. In other words, in~\cite{ben2016testing, haq2022efficient}, the objective is to generate individual test cases that can reveal the most severe failures. In contrast, our work  aims to develop failure models that explain when a failure occurs and when it does not.\\
Finally, we have made significant enhancements to our paper, addressing all the comments from the reviewers. The  improvements notably include:
\begin{enumerate}
\item Enhancing the readability  of Algorithms~\ref{alg:alg1}, \ref{alg:alg2}, \ref{alg:alg4}, \ref{alg:alg5} and \ref{alg:alhazen} by adding comments;
\item Introducing Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift} for a clearer visual representation of how Algorithm~\ref{alg:alg2} works;
\item Further clarifying  Algorithm~\ref{alg:alg2} by presenting it in a step-by-step manner. The details for Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift}, as well as the enhanced presentation of Algorithm~\ref{alg:alg2}, are available on~\referenceaddressed{R2C6l}.
\item Improving the clarity of Algorithms~\ref{alg:alg4} and \ref{alg:alg5} by adding examples;
\item Organizing Section~\ref{subsec:mainloop} into subsections, with each subsection focusing on a distinct approach;
\item Extending the``Threats to Validity'' section (Section~\ref{subsec:threats}) to address and discuss potential internal validity risks;
\item Providing clarification on the metrics used in RQ1 as well as additional details on RQ2 results.
\end{enumerate}}
%we have substantially improved the presentation of our paper and have addressed all the comments raised by the reviewers.  The specific improvements are as follows: (1) We have added comments to Algorithms~\ref{alg:alg1}, \ref{alg:alg2}, \ref{alg:alg4}, and \ref{alg:alg5} to improve readability and understanding. (2) We have introduced Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift} to offer a clearer visual representation of Algorithm~\ref{alg:alg2}'s operation.  (3) We have enhanced the presentation of Algorithm~\ref{alg:alg2} by illustrating and explaining it step by step. Descriptions for Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift} and the refined presentation of Algorithm~\ref{alg:alg2} can be found on~\referenceaddressed{R2C6l}. (4) We have improved clarity in Algorithms~\ref{alg:alg4}, and \ref{alg:alg5} by providing examples and detailed explanations. (5) We have divided Section~\ref{subsec:mainloop} into subsections, each corresponding to a specific approach.  (6) We have expanded the ``Threats to Validity`` section (Section~\ref{subsec:threats}) to cover and mitigate risks associated with internal validity. (7) We provided clarifications for the metrics in RQ1 and presented additional details for the results in RQ2.   
% FROM R1 Comment 3. 
%}


% \rwcomment{ARC2}{Journal First Definition}
% \response{}





\newpage

\noindent\textbf{Reviewer \#1} 

\rwcomment{R1C1}{I am not entirely convinced by the premise that test cases leading to spurious failures are really that useless as claimed by the authors. In contrast, this is what error testing and stress testing is all about: to ensure that the systems also reacts properly (i.e., to remain in a controlled state) in case of implausible inputs. For instance, even though it is invalid to have the input “airplane nose up” in combination with a certain other input value (according to the example described by the authors), we may think of cases where this might happen in practice (e.g., due to erroneous sensor data or unexpected data bus overload). Also in this case, it is important to ensure that the plane shows a proper reaction (e.g., ignoring implausible sensor data). If I remember it correctly, then something like this happened to the fatal Lion Air Flight 610 a few years back. I recommend discussing this issue in much more detail and to relax the assumptions about spurious failures, accordingly.
}
\response{We appreciate your comment and agree with your perspective.  We have added the following clarification on~\referenceaddressed{R1C1l}: It is essential for systems to handle all potential inputs including those that violate environment assumptions, and hence, are invalid. Spurious failures caused by invalid test inputs indicate a need for additional safeguards against invalid inputs that may be generated, among other sources, by human operator errors or malfunctioning hardware components, such as inaccurate sensor data.  However, these invalid test inputs do not exercise the core functionality of a system. While ensuring that a given system is safeguarded against invalid inputs is crucial, the inability to identify spurious failures can distort our understanding of the system's capabilities.  This may also lead to misplaced confidence in a testing strategy that reveals numerous failures, yet offers little insight into the system's primary functions.}

\rwcomment{R1C2}{In addition to the system under test itself, the approach further relies on additional knowledge about the system in terms of a fitness function for test cases and a specification of the input search space. It is unclear to me to what extent the accuracy of the learned rules depends on the quality of the the initial data sets. If this knowledge is inaccurate or even entirely missing or, what does this mean for the accuracy of the results? And, even more important, do I know as a user of the approach how reliable the derived decision rules are depending on my inputs? I would like to ask the authors to please elaborate some more on this serious threat to validity.}
\response{Thank you for your comment. We have extended the threats to validity section in~\referenceaddressed{R1C2l} to discuss the risks and our mitigation strategies related to the accuracy of fitness functions and the quality of input datasets. The newly added text reads as follows: The \textit{internal validity} risks are related to confounding factors.  The effectiveness of failure-inducing rules  inferred by our approach depends on the accuracy of fitness functions and the quality of the input datasets. For Simulink models, we use an automated and provably sound technique to obtain fitness functions from logical specifications~\cite{menghi2019generating}. However, the translation of natural-language requirements into logical specifications remains a manual task and necessitates domain-expert validation. In our experiments, we mitigated the risks associated with the accuracy of fitness functions as follows: For Simulink models, the fitness functions are automatically obtained from logical specifications approved by the engineers who developed the benchmark Simulink models~\cite{nejati2019evaluating}.  For the NTSS case study, we validated the fitness function in collaboration with our industry partner and against domain knowledge~\cite{enrich}. As for the risks related to the quality of datasets, we note that the labels for the dataset elements are computed  based on the actual system outputs, and hence, are always accurate. In addition,  we used adaptive random testing in the preprocessing step (see Figure~\ref{fig:fig1}) to diversify the generation of the datasets in the search input space.}


%We clarify that the main purpose of RQ1-2 is to  determine whether the re-executions of flaky tests represent fundamentally flawed scenarios, or whether, despite generating different fitness values, these re-executions still represent valid  driving scenarios. The conclusion is that among the 40 randomly selected flaky test samples, only one sample exhibits totally infeasible and flawed  reruns, and the reruns of the remaining  samples are reasonable and, independently, realistic. While RQ1-2 offers insights into the variations caused by the flakiness of simulator-based testing of ADS, we believe that it is not sufficient to draw conclusions on the root causes of flakiness solely based on the results presented in Table~\ref{tab:variations-carla}.

\rwcomment{R1C3}{The description of the algorithms in Section 3 is quite dense and often hard to follow. It would be helpful for the reader if the different steps would be further illustrated by concrete examples (e.g., using extracts from the code and test cases of the motivating examples described in Section 2 or at least using some small toy examples).}
\response{We have substantially improved the presentation of the algorithms in Section~\ref{sec:approach}. The specific improvements include:
\begin{enumerate}
\item Enhancing the readability  of Algorithms~\ref{alg:alg1}, \ref{alg:alg2}, \ref{alg:alg4}, \ref{alg:alg5} and \ref{alg:alhazen} by adding comments;
\item Introducing Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift} for a clearer visual representation of how Algorithm~\ref{alg:alg2} works;
\item Further clarifying  Algorithm~\ref{alg:alg2} by presenting it in a step-by-step manner. The details for Figures~\ref{fig:figalg2} and~\ref{fig:fitnessshift}, as well as the enhanced presentation of Algorithm~\ref{alg:alg2}, are available on~\referenceaddressed{R2C6l}.
\item Improving the clarity of Algorithms~\ref{alg:alg4} and \ref{alg:alg5} by adding examples;
\item Organizing Section~\ref{subsec:mainloop} into subsections, with each subsection focusing on a distinct approach;
\end{enumerate}}


%The specific improvements are as follows: (1) We added comments to Algorithms~\ref{alg:alg1}, \ref{alg:alg2}, \ref{alg:alg4}, and \ref{alg:alg5} to improve readability and understanding. (2) We introduced Figures~\ref{fig:figalg2} and \ref{fig:fitnessshift} with descriptions for a more visual illustration of how Algorithm 2 operates. (3) We improved clarity in Algorithms~\ref{alg:alg2}, \ref{alg:alg4}, and \ref{alg:alg5} by providing examples and detailed explanations. (4) We divided Section~\ref{subsec:mainloop} into subsections, each corresponding to a specific approach. (5) We renamed Section~\ref{subsec:fms} to clarify the purpose of this section. (6) We enhanced the figure captions.}
% @BHARIN: Please outline all the presentation improvements you have done for reviewer 2 here.  }


\newpage

\noindent\textbf{Reviewer \#2}

\rwcomment{R2C2}{It is not clear the contribution of this paper, as it is presented as journal first and there is no reference to previous work. So, please specify what is the new part compared to the conference paper.}
\response{Our paper reports completely new research results and  contributions that have not been reported in any previous work. In other words, our paper does not extend any existing paper. As such, our paper satisfies the conditions of the journal-first category. \\
In the manuscript, we present, for the first time,  a  data-driven framework for inferring failure models for systems with numeric inputs. This framework examines surrogate-assisted and machine learning-guided test generation techniques. We explore how effective these  techniques are at generating failure models. To our knowledge, this topic 
has not been studied before. We conclude by discussing  the limitations of  having testing focused exclusively on finding individual failures, and provide insights about the advantages of using failure models as a tool for measuring the effectiveness of testing algorithms.}


\rwcomment{R2C3}{Page 2 -> my first concern is about the definition of spurious failures. These failures are caused by inputs that do not satisfy pre-conditions. If your system has a pre-condition, why these values are given as input?
}
\response{Thank you for the comment. We have now clarified the definition of spurious failures by stating that they are caused by inputs that do not satisfy environment assumptions.  Environment assumptions capture the expected conditions for a system's operational environment~\cite{giannakopoulou2002assumption}. Attempting to test a system for a more general environment than its expected operational environment may lead to overly pessimistic testing and verification results.
We refer to failures arising from test inputs violating the system's environment assumptions as \emph{spurious failures}. It is often the case that environment assumptions are not fully known for software systems~\cite{10.1145/3270112.3270115}; therefore, it is difficult to determine whether a failure is indeed spurious. We have revised the definition of spurious failures on~\referenceaddressed{R2C3l}.}




\rwcomment{R2C4}{page 3, line 6 -> which is the difference between your work and references 32,49?}
\response{Thank you for the comment. We have now clarified on~\referenceaddressed{R2C4l} that \cite{ben2016testing} and \cite{haq2022efficient} pursue different goals and use different algorithms compared to ours. Specifically,  earlier work strands~\cite{ben2016testing, haq2022efficient} employ machine learning to more effectively steer test generation towards areas within the search space that are likely to contain the most severe failures. In this paper, we use machine learning to devise new test generation algorithms, with the aim of inferring failure models for systems that have numeric inputs. In other words, in~\cite{ben2016testing, haq2022efficient}, the objective is to generate individual test cases that can reveal the most severe failures. In contrast, our work aims to develop failure models that explain when a failure occurs and when it does not.} 

\rwcomment{R2C5}{page 7
line 24->you introduce SMOTE, but then you don't use it. 
line 31-> it is not clear to me
algorithm 1 -> is algorithm 1  the algorithm called as InitializeAndBalance in the other algorithms? If so, please give the same name to algorithm 1}
\response{We clarify that SMOTE is indeed used on line~3 of Algorithm~\ref{alg:alg1}. We have now added a comment to Algorithm~\ref{alg:alg1} to explicitly indicate which step of that algorithm uses SMOTE.  Specifically, we use SMOTE to generate synthetic test inputs by over-sampling the minority class. However, we discard the labels provided by SMOTE, since SMOTE categorizes test inputs as pass or fail. Instead, we require test inputs to be labelled with their quantitative fitness values; this enables us to train regression ML models in Step~$3$ of our approach in Figure~\ref{fig:fig1}. Provided with the fitness values, we can also compute accurate pass and fail labels for test inputs generated by SMOTE. We have added this clarification on~\referenceaddressed{R2C5l}.\\
%To compute the fitness value of each test input which is not calculated by SMOTE. The fitness value of each test input is required in the later steps to train an ML model.
%To ensure that the label assigned to each test input is accurate. If a label assigned by SMOTE is not correct, we overwrite it with the actual label. The labels of the test inputs will be used in Step~$5$ of Figure~\ref{fig:fig1} to build a failure model.
%\end{itemize}
%We have also added comments to Algorithm~\ref{alg:alg1} to show where SMOTE is used.
As for the second comment,  we have now replaced $\mathit{InitializeAndBalance}$ with $\mathit{Preprocessing}$ in Algorithms~\ref{alg:alg2}, \ref{alg:alg4},  \ref{alg:alg5} and \ref{alg:alhazen}. We have further added  comments to these algorithms to explicitly indicate that $\mathit{Preprocessing}$ refers to Algorithm~\ref{alg:alg1}.}

\rwcomment{R2C6}{page 8
line 31 -> "to obtain its predicted fitness value" -> could you explain better how do you do the prediction? algorithm 2 : could you better describe lines 3-6?what is "flag"? if the condition in line 9 is false, $DS^l$ is not updated, so in the next step SM and e are the same? Why do you have the condition in line 9? Why do you need it?}
\response{These comments are related to Algorithm~\ref{alg:alg2}. We have now added Figures~\ref{fig:figalg2}~and~\ref{fig:fitnessshift} to offer a clearer visual representation of Algorithm~\ref{alg:alg2}'s operation. Furthermore, we have enhanced the presentation of Algorithm~\ref{alg:alg2} by illustrating and explaining it step by step. Descriptions for these two new figures and the refined presentation of Algorithm~\ref{alg:alg2} can be found on~\referenceaddressed{R2C6l}.\\
Regarding the comment ``to obtain its predicted fitness value'', the predicted fitness values are outputs of the surrogate models. Surrogate models are denoted by $\mathit{SM}$ in Algorithm~\ref{alg:alg2}. We have now clarified on line~8 of Algorithm\ref{alg:alg2} that the predicted fitness value for a test input $t$ is obtained by passing the test input to  the surrogate model. This is indicated using a proper notation and a comment, with the prediction denoted as $\mathit{SM}(t)$. In addition, a clarification has been provided on~\referenceaddressed{R2C6PP}.\\
In response to the comment about the ``flag'' variable, we have added a visual clarification in Figure~\ref{fig:fitnessshift}. This figure demonstrates how the decision is made as to whether to run the system for a test input $t$ to determine its actual fitness value. The Boolean variable $\mathit{flag}$ represents  this decision: if $\mathit{flag} = \top$, the system is executed for test input $t$; if $\mathit{flag} = \bot$, it is not. When the system is executed for a particular test input $t$, the surrogate model is retrained, after updating its training dataset with this test input. In the absence of a new system execution, retraining the surrogate model is not necessary.\\
As you correctly point out, when $\mathit{DS}^l$ remains unchanged, $SM$ and $e$ are not updated. However, each iteration involves sampling a new test $t$, yielding a different value of the predicted fitness $\bar{F}(t)$. The decision to execute the system and potentially retrain the surrogate model is revisited for each new test input, as the confidence interval $\bar{F} \pm e$ varies. This is depicted in Figure~\ref{fig:fitnessshift}.\\
In view of the above explanation, the condition on line~$9$ is essential to determine whether a predicted fitness value is sufficiently accurate to make  a pass/fail verdict. If not, we execute the system for that input to obtain its actual fitness value and an accurate verdict. In the latter case, updating the training set $\mathit{DS}^l$ and retraining $\mathit{SM}$ becomes necessary.}


%Regarding the comment related to the ``flag" variable, we have a visual clarification using Figure~\ref{fig:fitnessshift}. As the figure shows, for a given sample $t$ we make a decision as to execute the system for $t$ to compute its actual fitness value based on the predicted fitness $\bar{F}$ and the error $e$ both of which are obtained from the surrogate model $\mathit{SM}$. The boolean $\mathit{flag}$ variable captures this decision, when $\mathit{flag} = \top$, we execute the system and when $\mathit{flag} =\bot$ we do not execute the system.  We only re-train the surrogate model when we execute the system with a new sample. Otherwise, without having any new execution, there is no need to retrain the surrogate model since $\mathit{DS}^l$  can only be updated if we have a new system execution. We note that as you have indicated when $\mathit{DS}^l$ is not changed, $\mathit{SM}$ and $e$ are not updated. However, in each iteration, we sample a new test $t$ and the predicted fitness of that sample $\bar{F}(t)$ is a different value. 

%The descriptions of these figures are in Section~\ref{sec:surrogate} (pages 7-9). Briefly, Algorithm~\ref{alg:alg2} starts by running Algorithm~\ref{alg:alg1} to generate an initial dataset (Step 1 in Figure~\ref{fig:figalg2}). Then, this dataset is used to train a surrogate model (Step~$2$) and compute its error ($e$). The surrogate models that we have used in our experiments are \emph{regression} models (see Table~\ref{tab:surrogatemodels}) and we use them to compute (i.e. predict) the fitness value of a test input. Next, we generate a random test input and use the surrogate model to compute its fitness value (Steps~$3$ and $4$). To determine whether the system needs to be executed or not, we shift the fitness value (Step~$5$). Specifically, we analyze whether adding (resp. removing) model error $e$ to (resp. from) the fitness value would change the test verdict from pass to fail or vice versa. If shifting the fitness value does not impact the test verdict, we add the test input and its fitness value to the dataset and do not execute the system (Step~$6$ after No branch). Therefore, the surrogate model and its error ($e$) will remain unchanged for the next iteration. Otherwise, we execute the system to compute the actual fitness value (Step~$6$ after Yes branch) and update the dataset by adding the test input along with its actual fitness value (Step~$7$). In this case, we re-train the surrogate model using the updated dataset. In our algorithm, we use $\mathit{flag}$ to determine whether we need to re-train a surrogate model or not (line~$4$). We note that we only train the surrogate model on the dataset where the fitness values are computed by executing the system (i.e. $DS^l$ in line~$5$). This is to ensure that the surrogate model is tailored to the actual fitness values rather than relying on predicted fitness values (i.e. fitness values computed by the surrogate model), which may introduce errors or uncertainties. }
% SM(t) not predict. Say that surrogate models are regression models. Create a figure for surrogate models. Baharin.

\rwcomment{R2C7}{page 9
line 26-27 -> in the algorithm there is a condition with "and", please rephrase accordingly 
line 30 -> which are the old $v_1,v_2,v_3$?}
\response{To improve the readability, we have now simplified the termination condition for the while loops of Algorithms~\ref{alg:alg2}, \ref{alg:alg4}, \ref{alg:alg5} and \ref{alg:alhazen}. Specifically, we now use a single condition, i.e., 
while (execution budget remains), instead of a conjunction of two conditions that we had before. We note that this simplification does not in any way impact the semantics of our algorithms. We have now improved the explanation of the termination condition on~\referenceaddressed{R2C7l}, \referenceaddressed{R2C7PP}, and \referenceaddressed{R2C7K}: 
The execution budget expires when either the system has been executed to the point where the size of $DS$ reaches its desired limit, or our time budget is exhausted, depending on which occurs first. \\
In response to the comment about $v_1$, $v_2$, and $v_3$, we refer to the example in Figure~\ref{fig:regtreeexample}.  This example clarifies how to update the ranges of variables appearing on the boundary paths, which are marked with thick, blue-highlighted lines. In this example, we assume that the old ranges for $v_1$, $v_2$ and $v_3$ are [0, 20], [10, 30], and [1, 7], respectively. The new reduced ranges obtained from the tree for $v_1$, $v_2$ and $v_3$ (i.e., $[9.5, 10.5]$, $[19, 21]$ and  $[4.75, 5.25]$, respectively) replace the old ranges. We have now clarified the old ranges of the these variables on \referenceaddressed{R2C7y}. }
% BAHARIN. NOT SURE WHAT THE PROBLEM IS. But in general the readability should improve. remove budget/2 from alg 4 and 5. time budget is set to half of the simulations. add ranges for v1, ...  }

\rwcomment{R2C8}{page 10, section 3.3 -> is this section about "Build failure model" in fig.1?}
\response{Yes, Section~\ref{subsec:fms} is about building failure models, i.e., Step~$5$ in Figure~\ref{fig:fig1}. We have now changed the title of Section~\ref{subsec:fms} from \emph{Input Feature Selection for Failure Models} to \emph{Building Failure Models} (see~\referenceaddressed{R2C8l}). This section discusses how we  prepare datasets and select input features to develop failure models using decision-rule algorithms.}   




% this section is about building failure model. change the section name to build failure model. it is important to do feature selection.}

\rwcomment{R2C9}{page 13, line 32-36 -> How do you count the number of incorrect labels?}
\response{Thanks for your comment. To obtain the actual fitness values for all test inputs, we run the system using those test inputs for which only surrogate-assisted algorithms provided predicted fitness values.
%we run the system on those test inputs for which only predicted fitness values were provided by the surrogate-assisted algorithms. 
Note that this step is intended exclusively for our experiments and is not a component of our main approach. Next, we count the number of tests in which the predicted label differs from the actual one.
The number of incorrectly labelled tests serves as a measure of error or inaccuracy for the surrogate-assisted algorithms. We have clarified this on \referenceaddressed{R2C9l}.} 
% for the purpose of experiments we execute the predicted tests.}

\rwcomment{R2C10}{page 14, fig.3 -> please check the scale
}
\response{Thank you for the comment. We have now increased the size of Figure~\ref{fig:rq1-1} and also carefully checked the $x$ and $y$ axes of the figure and their scales.}

\rwcomment{R2C11}{page 16 line 41 -> why the average reaches a plateau?}
\response{Thanks for this interesting comment. 
% Our random search algorithm (RS) randomly generates test inputs in the input space without any guidance or assistance from machine learning models. However, other approaches such as surrogate-assisted or ML-guided test generation leverage machine learning models to enhance their test generation. Specifically, surrogate-assisted technique uses surrogate models (machine learning models) to efficiently generate a substantial number of test inputs within a given time budget. On the other hand, ML-guided technique relies on machine learning models such as regression trees (RT) or logistic regression (LR) to identify and explore specific regions within the input space. 
The comment concerns Figure~\ref{fig:avgaccbudget} where the average accuracy of RS plateaus at the last two data points whereas the average accuracy of  the RT, LR and SA algorithms shows improvement for all the data points. The main reason for this difference is that RS, unlike the other algorithms, does not use machine learning models to guide its test input sampling.  Specifically, RS generates test inputs randomly across the entire input space. In contrast, RT and LR exploit boundary regions that separate passing and failing test inputs, resulting in a steady increase in accuracy as the search budget grows.  Further, SA utilizes surrogate models, generating significantly more test inputs compared to the other algorithms within the same allotted time budget. As a result, SA achieves the highest average accuracy among all the algorithms. We have now added this explanation on \referenceaddressed{R2C11l}.}




% In particular, within the range of 90\% to 100\% of the time budget, RS randomly generates test inputs from the input space, while RT and LR focus on exploiting a specific region within the input space. Although RS, RT, and LR each generate roughly the same number of test inputs, employing machine learning models to explore a specific region has a non-negligible effect on the average accuracies of RT and LR. Further, SA generates a higher amount of test inputs (compared to RS, RT and LR) between that time budget therefore it has the highest average accuracy.}
% is randomly      
% BAHARIN. RS randomly generates in space without any guidance/surrogate. but other approaches either exploit a specifc region . the difference betweeen 90\% and 100\% is e.g. 100 tests where RS generates them randomly but RT, LR exploit a specific region. SA generates more than 100.}


\rwcomment{R2C12}{page 20, algorithm 6 -> how do you guarantee that the algorithm exactly performed what is performed by SOTA?
}
\response{Thank you for your comment. As discussed on \referenceaddressed{R2C1211}, Alhazen~\cite{kampmann2020does}, i.e., SoTA, is designed mainly for systems with structured inputs, whereas  our focus is on systems with numeric inputs. 
However, since there are no existing baseline techniques designed specifically for generating failure models for numeric input systems, Alhazen is our best available baseline. We have adapted Alhazen to facilitate comparison, as detailed on \referenceaddressed{R2C1222}. The pseudo code for the adapted version is  provided in Algorithm~\ref{alg:alhazen}. Based on our comprehensive review of Alhazen's code~\cite{alhazengithub}, we confirm that the workflow of Algorithm~\ref{alg:alhazen} conforms to that of Alhazen. Furthermore, we employed the same hyperparameters for decision trees in Algorithm~\ref{alg:alhazen} as those used by Alhazen. To address your concern about a potential internal validity threat, we have included our response in the ``Threats to Validity'' section on~\referenceaddressed{R2C1233}.}


%We have compared our top-performing approach (i.e. SA) against state-of-the-art (SoTA). Alhazen~\cite{??} is the closest SoTA approach that we selected to compare our approach against. Since Alhazen~\cite{??} is geared towards systems with structured inputs, it is not immediately applicable to our systems (which have numeric inputs). Therefore, we conducted a thorough examination of Alhazen's code~\cite{alhazengithub} and re-implemented it so that it can be applied to our case studies. We have disclosed the code that we have implemented, in Algorithm~\ref{alg:alhazen} and in our GitHub repository~\cite{??}.} 
% we note that SOTA is not immediately applicable to our code. to disclose what we did we provided alg. 
% note to internal threat: in comparison with baseline: we defined our own baseline and checked their implementation and disclosed our algorithm.

\rwcomment{R2C13}{page 20 -> it is not clear the connection between usefulness of failure models in identifying spurious failures.}
\response{Thank you for the comment. We have now clarified on~\referenceaddressed{R2C13l} that, according to the description of RQ4, our objective is to evaluate the usefulness of failure models in identifying spurious failures.}

\newpage

==> Sections/assumption.tex <==


%Each $v_i$ can be a float or an enumerate variable. A float variable $v_i$ takes its values from a continuous interval $[a_i..b_i] \subset \mathbb{R}$, and an enumerate variable $v_i$ takes its values from a set $\{a_i,\ldots, b_i\} \subset \mathbb{N}$. As we will show later,  complex CPS inputs (e.g., time series and signals) can be encoded in terms of a few float  or enumerate variables. 


%\textbf{A2.} \emph{We assume that test inputs are executed on the system using a simulator, and test outputs are generated by the simulator.}  Let $\bar{v}$ be a test input. By simulating $\bar{v}$, we obtain $\bar{u} = (u_1, \ldots, u_m)$ as the test output. We note that we do not make any assumptions on the structure and type of output variables $u_1$, \ldots, $u_m$. Output variables can be of any type or structure. As we will see later, for cyber-physical models, output variables can be represented using signals. 




%There is a fitness function for $S$ that, for each test input executed against $S$, the oracle function provides a quantitative fitness measure from which a pass/fail verdict can be derived. Let $\mathcal{O}$  be a  test oracle  function, and let $t$ be a test input. Then, $\mathcal{O}(t)$ is a quantitative value in $\mathbb{R}$ that differentiates between the pass and fail verdicts. That is, there is threshold $\mathit{th}$ such that  $\mathcal{O}(t) \geq \mathit{th}$  iff $t$ is passing, and otherwise, $t$ is  failing. 





%http://crest.cs.ucl.ac.uk/cow/51/slides/cow51_verel_2.pdf
%http://crest.cs.ucl.ac.uk/cow/51/

%https://www.georgejpappas.org/papers/RV06.pdf

%In a nutshell, NTSS works as follows~\cite{??}: NTSS divides the available bandwidth into a number of classes with different bandwidth thresholds and priorities. Network data flows are assigned to these classes based on the NTSS internal configuration. The idea is to configure NTSS such that it assigns the time-sensitive, streaming voice and video applications to the classes with a higher priority. The higher priority classes aim to transmit the data flows  with lower latency compared to the lower priority classes. Note that the high priority classes guarantee the low latency only up to their threshold bandwidth. Hence, the latency of high priority classes may deteriorate if the total bandwidth of the data flows going through the high priority classes exceed the threshold. This policy ensures that the lower priority classes are not starved by the higher priority ones. 



%Configuring NTSS, i.e., assigning different data flow types to different priority classes and setting the classes' bandwidth thresholds, poses a challenge due to the complexity of the internal algorithms of NTSS and the users' unknown traffic usage profiles. For example, if a high priority class of NTSS is stressed since users launches several streaming applications in parallel, the quality of the transmission in that class can sharply deteriorate, leading to interrupted calls and videos. Knowing the characteristics of the traffic usage profiles that lead to low quality transmission can greatly assist engineers to configure NTSS effectively. 







==> Sections/goal1.tex <==
% \usepackage{multirow}
\begin{table}[t]

\caption{Input Features that appeared in the datasets}
\label{tab:goal1}
\scalebox{0.56}{ \begin{tabular}{|l|l|l|}
\hline
\textbf{Case Study}        & \textbf{Rule}                         \\ \hline
\multirow{4}{*}{Autopilot} & $\mathit{PitchWheel}[0...300] \leq -28.4 \land \mathit{Throttle}[0...300] \leq  0.1$                 \\ \cline{2-2} 
                           & $-28.1 \leq \mathit{PitchWheel}[0...300] \leq -22.1 \land 5.4 \leq \mathit{TurnKnob}[0...300] \leq 11 \land \mathit{ALTMode}[0...300] = 0 $                                          \\ \cline{2-2} 
                           & $\mathit{PitchWheel}[0...300] \leq -29 \land \mathit{ALTMode}[301...500] = 0$                                          \\ \cline{2-2} 
                           & $\mathit{PitchWheel}[0...300] \leq -28.6 \land \mathit{PitchWheel}[301...500] \leq -28.6$                                                       \\ \hline
NTSS      & $\mathit{Class5} + \mathit{Class6} + \mathit{Class7} \geq 75\% \cdot \mathit{maxClassRanges}$                                               \\ \hline 
                                      
\end{tabular}}
\end{table}

==> Sections/goal2.tex <==
%this one is with having the "feature" column:
%\begin{table}[t] 
%\label{tab:goal2}
%\caption{??}
%\scalebox{0.7}{
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Case Study}} & \multirow{2}{*}{\textbf{Feature}}       & \textbf{SA}            & \textbf{RS}            & \textbf{LogReg}  & \textbf{RegTree} \\ \cline{3-6} 
%                                     &                                         & \textbf{DT - DR}       & \textbf{DT - DR}       & \textbf{DT - DR} & \textbf{DT - DR} \\ \hline
%Autopilot                            & ALTMode, TurnKnob, PitchWheel, Throttle & (100, 45) - (100, 9)   & (100, 28) - (100, 6)   & ? / ?            & ? / ?            \\ \hline
%NTSS                                 & Class5 + Class6 + Class7                & (100, 37) - (96.3, 38) & (100, 32) - (99.6, 18) & ? / ?            & ? / ?            \\ \hline
%\end{tabular}}
%\end{table}

\begin{table}[t]

\caption{Comparing confidence and support values of four techniques for DT and DR}
\label{tab:goal2}
\scalebox{0.79}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Case Study}} & \textbf{SA}            & \textbf{RS}            & \textbf{LogReg}  & \textbf{RegTree} \\ \cline{2-5} 
                                     & \textbf{DT - DR}       & \textbf{DT - DR}       & \textbf{DT - DR} & \textbf{DT - DR} \\ \hline
Autopilot                            & (100, 45) - (100, 9)   & (100, 28) - (100, 6)   & ? - ?            & ? - ?            \\ \hline
NTSS                                 & (100, 37) - (96.3, 38) & (100, 32) - (99.6, 18) & ? - ?            & ? - ?            \\ \hline
\end{tabular}}
\end{table}

==> Sections/letterMajorReview.tex <==
\hfill\today

\vspace{1cm}

\noindent Dear Editor,

\vspace{1cm}


\noindent Enclosed please find a revised version of manuscript  \textbf{TOSEM-2023-0178}, titled \emph{``Test Generation Strategies for Building Failure Models and Explaining Spurious Failures''}. The manuscript is authored by 
Baharin A. Jodat (University of Ottawa), 
\hbox{Abhishek Chandar} (University of Ottawa),
\hbox{Shiva Nejati} (University of Ottawa), and
\hbox{Mehrdad Sabetzadeh} (University of Ottawa). 
We submitted the first version of the manuscript in June 2023.\\

In October 2023, we received a decision regarding the manuscript, indicating that a major revision was required. We are grateful to the reviewers for their excellent suggestions for improvement. We believe we have addressed all of the reviewers' comments as we detail in our responses provided alongside this letter.\\



\noindent In our responses,  each comment is followed by an explanation which is either a clarification or a description of the  changes we have made in the manuscript to address the comment.
The comments are highlighted in \textcolor{red}{red}, while our responses are highlighted in \textcolor{blue}{blue}.\\ %We indicate \emph{how} and \emph{where}  each comment has been addressed in the manuscript. \\

We identify each comment in the manuscript with a label in the format \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize Cn}, where n is an incremental number used for reference  in the manuscript.\\

\noindent For clarity, we attach a version of the manuscript where changes are  highlighted in \textcolor{blue}{blue}.  \\


%\vspace{1cm} 

\noindent Thank you for considering our manuscript.\\[2em]
 \noindent
Sincerely,\\[.5em]
Baharin A. Jodat, \hbox{Abhishek Chandar},  \hbox{Shiva Nejati}, \hbox{Mehrdad Sabetzadeh}
\clearpage

==> Sections/oldstuff.tex <==

\begin{minipage}{.9\linewidth}
%\vspace{-1cm}
\begin{algorithm}[H]
%\algsetup{linenosize=\scriptsize}
\scriptsize
\caption{Surrogate-Assisted Test Generation.}
\label{alg:overallalgorithm}
\begin{flushleft}
\textbf{Inputs}. $\mathit{S}$: Simulator or (executable) system \hfill \\
 \hspace{0.65cm}  $(R_1, \ldots, R_n)$: The search space \\
 \hspace{0.65cm}  $\mathcal{O}$: Test oracle function  \\
 \textbf{Outputs}. $\mathit{DS}$: A test data set\\ 
 \end{flushleft}
\begin{algorithmic}[1]
\Function{$A$=SAGACIOUS}{$\mathit{Sys}$, $(R_1, \ldots, R_n)$, $\mathit{pfThresh}$, $opt$, $\textsc{Budget}$}
\State \hspace{-0.3cm} $i$ = $0$; $TS = []$; $R = (R_1, \ldots, R_n)$  \Comment{Variables Initialization}
\State \hspace{-0.3cm} $TS$, flag= \Call{GenTests}{$\mathit{Sys}$, $opt$, $R$, 'SIM', $\mathit{pfThresh}$} \Comment{Test input generation and simulation} %initial number of test cases to be generated is passed in opt.
%\State \hspace{-0.3cm} TSAll = TS;
\State \hspace{-0.3cm} $M$ = \Call{BuildSurrogate}{$TS$, $opt$}; \hspace{-.3cm} \Comment{Build a surrogate model (ensemble or individual)}
\State \hspace{-0.3cm} \textbf{while} ($i  < \textsc{Budget}$)
\State \hspace{-0.28cm} \hspace{0.1cm} $tc$, flag = \Call{GenSingleTest}{$\mathit{Sys}$,$M$, $opt$, $R$, $\mathit{pfThresh}$}; \Comment{Test input generation using simulation or prediction}
\State \hspace{-0.28cm} \hspace{0.1cm} $TS$ = $TS$ $\cup \ tc$; \Comment{Combine new and old tests}
\State  \hspace{-0.28cm} \hspace{0.1cm}  $i$++; \Comment{Increases the counter}
\State  \hspace{-0.28cm} \hspace{0.1cm} \textbf{If} flag == 'SIM' \Comment{Check if the fitness of the test input is calculated by simulation}
\State  \hspace{-0.28cm} \hspace{0.1cm} \hspace{0.1cm} $M$ = \Call{BuildSurrogate}{$TS$, $opt$}; \hspace{-.3cm} \Comment{rebuild the surrogate model}
\State  \hspace{-0.28cm} \hspace{0.1cm}  \textbf{End If}
\State \hspace{-0.3cm} \textbf{EndWhile}
\State \hspace{-0.3cm} $DT$ = \Call{BuildDT}{$TS$, $opt$}; \hspace{-.3cm} \Comment{Build a decision tree}
\State \hspace{-0.3cm} $A$ = \Call{GenAssumption}{$DT$, $opt$}; \Comment{Assumption Generation}
\State \hspace{-0.3cm} \Return $A$;
\EndFunction
\end{algorithmic}
\end{algorithm}
\vspace{0.1cm}
\end{minipage}



\begin{table}[t]
\caption{The parameters required by \ourtool\ }
\label{tab:options}
\vspace{-.15cm}
\scalebox{0.6}{
\begin{tabular}{|l|p{3cm}|p{3cm}|p{3cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Step}} & \multicolumn{1}{|c|}{\textbf{Parameter}} & \multicolumn{1}{c|}{\textbf{Definition}}                         & \textbf{Value} \\ \hline
$Initial Sampling (Step 1)$ & \tabitem $\mathit{opt.PreNumPoints}$ \newline \tabitem  $\mathit{opt.TotalInitialPoints}$                                & \tabitem The preliminary points to generate and simulate  \newline \tabitem The total number of points to generate and simulate at step 1                                & \tabitem 150  \newline \tabitem 300         \\ \hline
$Balancing (Step 1)$ & \tabitem $\mathit{opt.SamplingStrategy}$ \newline \newline \tabitem $\mathit{opt.Kneighbors}$ \newline \newline \tabitem $\mathit{opt.Remaining}$                       & \tabitem The sampling strategy to use \newline \tabitem Number of nearest neighbours to us to construct samples \newline \tabitem Generate the remaining points       & \tabitem $minority$ \newline \newline \tabitem $2$ \newline \newline \tabitem  $??$        \\ \hline
$Second Loop (Step 2 \& 3)$ & \tabitem $\mathit{opt.MaxSimNum}$ \newline \tabitem $\mathit{opt.MaxIterNum}$ \newline \tabitem $\mathit{OptimizationMethod}$ \newline \tabitem $\mathit{opt.TestSize}$ \newline \tabitem $\mathit{ErrorMetric}$                             & \tabitem Maximum number of simulations \newline \tabitem Maximum number of iterations \newline \tabitem The hyper-parameter optimization method \newline \tabitem The size of the testset \newline \tabitem The metric used for calculating the error of a surrogate model      & \tabitem $300$ \newline \tabitem $3500$ \newline \tabitem Bayesian Optimization \newline \tabitem $20\%$ \newline \tabitem Mean Absolute Error              \\ \hline

\end{tabular}}
\vspace{-.3cm}
%\setlength{\textfloatsep}{-2cm}
\end{table}

\begin{table}[]
\scalebox{0.45}{
\begin{tabular}{|l|l|l|llll|}
\hline
\multirow{2}{*}{\textbf{Simulink Model}} & \multirow{2}{*}{\textbf{Description}} & \multirow{2}{*}{\textbf{Requirement}} & \multicolumn{4}{c|}{\textbf{Specifications}}                                                                                                         \\ \cline{4-7} 
                                &                              &                              & \multicolumn{1}{l|}{\textbf{\# inputs}}          & \multicolumn{1}{l|}{\textbf{\# control points}}   & \multicolumn{1}{l|}{\textbf{Fitness range}} & \textbf{Fitness threshold} \\ \hline
\multirow{2}{*}{Autopilot}      & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}A full six degree of freedom simulation of a single-engined \\ high-wing propeller-driven airplane with autopilot\end{tabular}}    & R1.4.1                       & \multicolumn{1}{l|}{\multirow{2}{*}{7}} & \multicolumn{1}{l|}{\multirow{2}{*}{21}} & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R1.6                         & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \hline
Regulator                       & A typical PID controller                     & R7                           & \multicolumn{1}{l|}{16}                 & \multicolumn{1}{l|}{16}                  & \multicolumn{1}{l|}{}              &                   \\ \hline
\multirow{9}{*}{Tustin}         & \multirow{9}{*}{A numeric model that computes integral over time}    & R1a                          & \multicolumn{1}{l|}{\multirow{7}{*}{4}} & \multicolumn{1}{l|}{\multirow{7}{*}{14}} & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R1b                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R1c                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R1d                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R1e                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R2a                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R2b                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \cline{3-7} 
                                &                              & R4a                          & \multicolumn{1}{l|}{\multirow{2}{*}{3}} & \multicolumn{1}{l|}{\multirow{2}{*}{3}}  & \multicolumn{1}{l|}{}              &                   \\ \cline{3-3} \cline{6-7} 
                                &                              & R4b                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}              &                   \\ \hline
\end{tabular}}
\caption{\label{tab:req}Simulink models and requirements used for experimentation}
\end{table}

Surrogate models (also known as approximation models or metamodels) are commonly used as alternatives to computationally expensive and costly simulators. Such models are estimating models that approximate the simulator's output for a given input. In this paper, we use surrogate models to approximate the fitness of a test input. Surrogate models need to achieve an acceptable level of accuracy before being utilized as a substitute for the actual simulator. 
The need for utilizing Surrogate models is growing in different domains. For example, surrogate models are used for approximating fitness function in evolutionary algorithms \cite{}, modelling the complex behaviour of agent-based models \cite{} and engineering design \cite{}. 
In addition to being computationally efficient, surrogate models are used as a verification and testing approach to identify system failures early and when they are less expensive to fix. For instance, Abdessalem et al. \cite{??} used surrogate models for Advanced Driver Assistance Systems (ADAS) to observe critical behaviours.
Commonly used surrogate models are Neural Networks, Support Vector Machine (SVM), boosting algorithms such as LS-boost, Gaussian Process Regression (Kriging), Regression Tree and Random Forest. These models can be used solely or in an ensembled way to predict the output of the simulator.

\textbf{Ensemble of Surrogate Models.} Choosing an appropriate surrogate model for a problem is difficult. Therefore, an ensemble of surrogate models is known to be a reasonable solution \cite{} and a way of having a reliable fitness prediction. The goal of this approach is to linearly combine surrogate models such that the impact of a poor surrogate model on the final fitness prediction is reduced. Particularly, for a test input $t$, the prediction of an ensemble model is a weighted summation of the predictions of individual surrogate models:

$\mathcal{R}_{ens}(t) = \sum_{i = 1}^{k} \mathcal{R}_i(t)\mathit{w_i}$ 

where $k$ is the number of surrogate models, $\mathcal{R}_i(t)$ is the fitness prediction of surrogate model $i$ for test input $t$ and $\mathit{w_i}$ is the weight assigned to surrogate model $i$. As a result, an important step in constructing an ensemble model is the selection of weights. Typically, surrogate models with higher (resp. lower) accuracies are associated with larger (resp. smaller) weights. To assign weights systematically, we propose a linear programming approach that aims to \emph{minimzie} the error of the prediction of an ensemble model. Specifically, the error of an ensemble model is calculated by
$\mathit{e_{ens}} = \sum_{i = 1}^{k} \mathit{e_i}\mathit{w_i}$ where $k$ is the number of surrogate models, $\mathit{e_i}$ and $\mathit{w_i}$ are the test error and weight assigned to surrogate model $i$, respectively. As a result, the goal is to minimize $\mathit{e_{ens}}$ such that (1) $\sum_{i = 1}^{k} \mathit{w_i} = 1 $, (2) $\mathit{w_i} \geq 0$, (3) $\mathit{w_i}\mathit{e_i} \leq \mathit{w_{i+1}\mathit{e_{i+1}}}$ with the assumption that the test errors $e_1, \ldots, e_k$ are in descending order. We use Matlab function \textsc{nma\_simplex} \cite{??} to solve this linear programming problem (i.e. calculate weights). The test errors $e_1, \ldots, e_k$ can be the average of Mean Absolute Error (MAE), Mean Squared Error (MSE) or Cross-Validation Error calculated based on the test suite.


I think here we need to define the notation for surrogate models. Discuss the main candidate for surrogate models as well as the idea of ensemble. 







An overview of \ourtool\ is shown in Figure~\ref{fig:overallapproach}.  \ourtool\ is implemented by Algorithm~\ref{alg:overallalgorithm} and performs the following tasks: (1) Generating and simulating a set of test inputs $(\mathit{TS_1})$ within a given search space, (2) Training a surrogate model on the test Suite $(\mathit{TS_1})$, (3) Generating test inputs $(\mathit{TS_2})$ and simulating or predicting their fitness, (4) Building a decision tree model based on $(\mathit{TS_2})$ and inducing an assumption such that test cases generated based on this assumption are likely to fail. The input of SAGACIOUS is a simulator,  $\mathit{Sys}$ (an instance of Simulink or NTSS), input ranges $R_1, \ldots, R_n$, pass/fail  threshold ($\mathit{pfThresh}$), and the required parameters bundled as $\mathit{opt}$ and detailed in Table~\ref{tab:options}.






\textbf{Step 1. Test Generation and Simulation.} The goal of this step (line 3 of Algorithm~\ref{alg:overallalgorithm}) is to generate and simulate a set of test inputs $(\mathit{TS_1})$ with size $\mathit{opt.TotalInitialPoints}$ within the search space. That is, we first randomly generate a set of test inputs ($\mathit{opt.PreNumPoints}$) within the given search space and calculate their fitness by simulating the test inputs. Further, we also label each test in the test suite as Fail or Pass based the pass/fail threshold provided by the domain knowledge. Specifically, tests whose fitnesses are greater (resp. smaller) than the threshold are considered as Pass (resp. Fail). In other words, for a test input generated in this step, we record both the fitness as well as the label. The labeled test suite will be used in Step 4 (Model Building) to generate an assumption for the input variables such that test inputs respecting that assumption likely fail. We note that since the tests generated in this step may be skewed to one of the classes (i.e. Fail or Pass), we use a frequently used method called Synthetic Minority Over-sampling Technique (SMOTE) \cite{??} to sample the minority class and balance the test suite. SMOTE first selects a minority class test $a$ randomly and finds its $k$ nearest neighbors ($\mathit{opt.Kneighbors}$). Afterwards, SMOTE randomly selects one of the $k$ closest neighbours (i.e. $b$), and joins $a$ and $b$ to construct a line in the feature space. A new synthetic test is then a point on this line \cite{??}.
%https://www.amazon.com/dp/1118074629/ref=as_li_ss_tl?&linkCode=sl1&tag=inspiredalgor-20&linkId=615e87a9105582e292ad2b7e2c7ea339&language=en_US
However, the fitness value of the synthetic tests generated by SMOTE may not be accurate. Therefore, we simulate these tests to retrieve their actual fitness value and label. Finally, for the remaining tests ($\mathit{opt.TotalInitialPoints} - ( \mathit{opt.PreNumPoints} + \mathit{SMOTE})$) we randomly generate and simulate tests to reach total of  $\mathit{opt.TotalInitialPoints}$ tests.



\textbf{Step 2. Train a Surrogate Model.} The goal of this step is to use the generated test suite of the first step $(\mathit{TS_1})$ to build a surrogate model (line 4 of Algorithm~\ref{alg:overallalgorithm}). The surrogate model can be a linear or non-linear machine learning model or an \emph{ensemble} of various machine learning models. We consider both linear and non-linear machine learning models since the interaction between input variables are unknown for us. In this step, we do not use the labels of the tests to train a machine learning model since our primary goal is to build an accurate surrogate model that can predict the fitness of a test input with a negligible error and therefore is an alternative to the compute-intensive simulator. As a result, we prefer machine learning regression models over classification ones to predict the fitness of tests in the later steps. The regression models that we utilize are Support Vector Regression (SVR), Regression Tree, Random Forest, LS-Boost, Gaussian Process Regression (GPR) and Neural Networks. We train the surrogate model (individual or enemble) on $\mathit{TS_1}$ and calculate its test error on a separate test set. 
%The ensemble of different regression models has been widely used as a way of having a reliable fitness prediction of a test input \cite{???}. Specifically, an ensemble of regression models is reliable as it aims to reduce the impact of a poor regression model on the final fitness prediction. Particularly, for a test input $t$, the prediction of an ensemble model is a weighted summation of the predictions of regression models:

%$\mathcal{R}_{ens}(t) = \sum_{i = 1}^{k} \mathcal{R}_i(t)\mathit{w_i}$ 

%where $k$ is the number of regression models, $\mathcal{R}_i(t)$ is the fitness prediction of regression model $i$ for test input $t$ and $\mathit{w_i}$ is the weight assigned to regression model $i$. As a result, an important step in constructing an ensemble model is the selection of weights. Typically, regression models with higher (resp. lower) accuracies are associated with larger (resp. smaller) weights. To assign weights systematically, we propose a linear programming approach that aims to \emph{minimzie} the error of the prediction of an ensemble model. Specifically, the error of an ensemble model is calculated by
%$\mathit{e_{ens}} = \sum_{i = 1}^{k} \mathit{e_i}\mathit{w_i}$ where $k$ is the number of regression models, $\mathit{e_i}$ and $\mathit{w_i}$ are the test error and weight assigned to regression model $i$, respectively. As a result, the goal is to minimize $\mathit{e_{ens}}$ such that (1) $\sum_{i = 1}^{k} \mathit{w_i} = 1 $, (2) $\mathit{w_i} \geq 0$, (3) $\mathit{w_i}\mathit{e_i} \leq \mathit{w_{i+1}\mathit{e_{i+1}}}$ with the assumption that the test errors $e_1, \ldots, e_k$ are in descending order. We use Matlab function \textsc{nma\_simplex} \cite{??} to solve this linear programming problem (i.e. calculate weights). The test errors $e_1, \ldots, e_k$ can be the average of Mean Absolute Error (MAE), Mean Squared Error (MSE) or Cross-Validation Error calculated based on the test suite generated in the first step ($TS_1$).


\textbf{Step 3. Test Generation using Simulation and Prediction.} This step (line 5 to 12 in Algorithm~\ref{alg:overallalgorithm}) generates test inputs within the given range with one main difference from step one. In this step, we use the surrogate model trained in the second step to predict the fitness of the generated test input. However, the prediction of the surrogate model might not be reliable or accurate enough. Assume that the predicted fitness for test input $t$ is $\mathcal{R}{(t)}$ and the error of the surrogate model is $e$. To check the reliability of the prediction, we further investigate the labels (Fail or Pass) of $\mathcal{R}{(t)} + e$,  $\mathcal{R}{(t)} - e$ and $\mathcal{R}{(t)}$. If all three labels are the same, then the prediction is reliable and we label the test input. Otherwise, we need to simulate the test input and label it again. The reason that we do it in this way is that the predicted fitness may deviate from the simulated fitness by an error margin (i.e. $e$). As a result, we explore whether or not by adding or deducting the error, the label of the test input changes. The test input is then returned by \textsc{GenSingleTest} (line 6 in  Algorithm~\ref{alg:overallalgorithm}) and is added to the test suite (line 7). In line 6, \textsc{GenSingleTest} also returns a boolean variable (i.e. $\mathit{flag}$) to indicate that the fitness of the generated test input is predicted (0) or simulated (1). We will later use $\mathit{flag}$ in line 10 to retrain the surrogate model if the fitness of the test input was retrieved by simulation (i.e. the value of flag is 1) since retraining the surrogate model on the predicted test may not be logical and it may even result in drop in accuracy of the surrogate model. This process continues until the budget runs out. 



%we are not building decision tree here

%\textbf{Step 4. Model Building.} This step shown in lines 13 and 14 of Algorithm~\ref{alg:overallalgorithm} builds a decision tree model on the test suite generated in step 3 ($\mathit{TS}_2$) and uses it to obtain an assumption such that test cases generated based on this assumption are likely to fail. We consider an interpretable machine learning model to produce comprehensive predicates from the tree. That is, we use the same state-of-the-art method in \cite{rabbitrunpaper} to extract a constraint based on input variables. That is, we use a decision tree model because its tree style structure allows us to compare and sort the tree paths. However, instead of regression tree which is used in \cite{rabbitrunpaper}, we employ a classification tree since our data is labeled Fail or Pass. A classification tree recursively splits each node of the tree into two child nodes until (1) the data in each node is homogeneous enough (i.e. the majority of the tests are labeled either Fail or Pass), or (2) each node satisfies the specified minimum node size. As shown in Figure~\ref{fig:decisiontreeexample}, each leaf node represents the probability of the classes (i.e. Fail or Pass) of the test cases in that node. Moreover, each edge in the tree is designated with a predicate in the form of $v_i \sim c$ where $v_i$ is an input variable, $c \in \mathbb{R}$ and $\sim \in \{\leq, >\}$. For example, in Figure~\ref{fig:decisiontreeexample}, the path that traverses nodes 1, 2, 5 and 9 corresponds to constraint $(v_1 \leq 10) \land (v_2 > -1) \land (v_3 > 51)$. In addition, a test scenario that satisfies this constraint is $93\%$ Fail and $7\%$ Pass. Next we explain how we extract a constraint (an assumption) from a path of the tree (line 14 of Algorithm~\ref{alg:overallalgorithm}). We start by extracting all the paths from the classification tree and sort the paths based on the probability of the Fail class in their leaf node. We then choose a path ($P$) that has the highest Fail class probability. 
%We note that we set the minimum node size ($\mathit{opt.MinNodeSize}$ in Table~\ref{tab:options}) to a value greater than one so that our sorting is meaningful and we don't end up comparing paths that there is a drastic difference between the number of test cases satisfying those paths.
%If there is more than such path, we choose the longer path, that is, the path with more distinct variables. The reason is that a path containing more distinct variables provides more predicates on input variables and as a result more variables are constrained. In the example of Figure~\ref{fig:decisiontreeexample}, path $P:$ (1, 3, 7, 10, 14) is chosen as it has the highest Fail probability (i.e. $75\%$). 
%The assumption induced by this path can now be used for test generation. 




%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/decisiontreeexample.pdf}
%    \imagecaptionspace
%    \caption{A decision tree generated by our approach and induced input ranges}\label{fig:decisiontreeexample}
%    \vspace{-.15cm}
%\end{figure}








\begin{itemize}
    \item We start by first considering subsets of the input variables as input features to our failure-inducing models i.e. decision tree and decision rules.
    \item For the NTSS case study, we consider the summation of the subset of the input variables as the input to the failure-inducing models.
    \item We use the data from the best approach (i.e. SA dynamic) in RQ1 to build FIMs for the subsets of the inputs. 
    \item We get the rules from FIMs that lead to failure, i.e. we find the rules of the form IF CONDITION THEN FAILURE. Each rule has a confidence $\mathit{conf}$ and a support $\mathit{sup}$ meaning that the label of what percentage ($\mathit{conf}$) of the tests holding the condition of the rule  ($\mathit{sup}$) is actually failure.
    \item For each feature (i.e. subset of input variables), we find the rules that have the highest confidence (i.e. $\mathit{conf}$). Then, among these rules we select the rules that have highest number of support (i.e. $\mathit{sup}$). We also find the number of rules whose confidence value is $100\%$.
    \item We repeat this process for all the runs. Finally, for each run, we choose the features that have the highest confidence and highest support. In this way, for each run we can determine the feature that explains the failure more confidently and supportively.
    \item Table~\ref{tab:?} shows a part of the features and ??. As can be seen in the table, for the Autopilot case study, by passing $\mathit{ALT Mode}$, $\mathit{Turn Knob}$, $\mathit{Pitch Wheel}$ and $\mathit{Throttle}$ to the decision tree, on average, we get the highest confidence and support. This means that these four inputs are the most effective inputs in failing the requirement. We have checked the documentations of the autopilot in \cite{??} and found out that $\mathit{ALT Mode}$ indicates that altitude of the aircraft is maintained by the autopilot, $\mathit{Turn Knob}$ indicates the roll angle of the aircraft, $\mathit{Pitch Wheel}$ refers to the control of the aircraft's nose in relation to the natural horizon and $\mathit{Throttle}$ refers to the power provided by the pilot.
    \item For the NTSS case study, $\mathit{Class5} + \mathit{Class6} + \mathit{Class7} > C$ is the most supportive and confident input feature for both decision tree and decision rules. We have checked the configuration of the NTSS with the domain expert and realized $\mathit{Class5}$, $\mathit{Class6}$ and $\mathit{Class7}$ are the highest priority classes and time-sensitive applications are mapped to these classes. The value of $C$ is around $390$ which is close to the total bandwidth that we have set for our experiments (see section~\ref{??}). Specifically, the value of $C$ indicates that when all the available bandwidth is dedicated to the highest priority classes, then the quality of the network will be low. 
    \item We have also compared the values of the confidence and support of the most effective feature from Table~\ref{tab:??} for dynamic approach with those of random search (Table~\ref{??}). As can be seen in this table, overall, for both case studies, the rules generated by SA dynamic approach are more supportive than the rules generated by random search. 
\end{itemize}



In this research question, we show how we infer rules characterizing failures from our failure models. For this research question, we use the datasets obtained by the best algorithm from RQ2 (i.e, SA). We focus on our two CI subjects form Table~\ref{tab:simulinkmodels} since they represent entire systems as opposed to components within larger systems and for these two we either have access to domain experts or public documentation.


DT and DR produce rules that are conjunctions of predicates where each predicate involves at most one variable. Since such rules may not be powerful enough to express conditions that concern more than one variable, for each case study, we need to design input features based on which we build failure models. Therefore, we propose the process in Figure~\ref{fig:RQ3Process} to extract rules from our failure models. 
Both autopilot and NTSS case studies have eight inputs.
Two of the inputs for autopilot are explicitly assigned to fixed values  in the formalization of the requirement (e.g., AP HAS TO BE ON IS a pre-requires of the requirement). For autopilot, we want to know which combinations of the remaining six variables can explain failure with the highest confidence. Therefore, as input features, we consider all 64 subsets. We then create 64 failure models, i.e., one for each subset, such that the input features of each failure model are the variables in the given subset. 

For NTSS, we consider the $255$ (i.e., $2^8-1$) subsets of the variables as input features. As discussed in Section~\ref{sec:motivation}, the purpose is to identify the bandwidth limits that the combination of NTSS classes  can take without compromising the network quality. Hence, we create 255 failure models, i.e., one for each subset. However, since in this case we are interested in the limit on the accumulation of the traffic going through different classes, we use a summation of variables in each subset as the input feature. 


Both DR and DT generate a set of rules in the form \textsc{IF-condition-THEN-prediction}, where condition is a constraint over the input features and prediction is either pass or fail. From each failure model, we extract rules with  the fail prediction. Each rule comes with two metrics: confidence and support. Support ($\mathit{sup}$) shows the number of tests that satisfy the condition of the rule, and confidence ($\mathit{conf}$) shows what percentage of support has fail labels. For example, \textsc{IF Class6 + Class7 $>$ 300 THEN FAIL} has $\mathit{conf} = 100\%$ and $\mathit{sup} = 20$. This means that $20$ tests satisfy the condition of this rule, and all the $20$ tests have fail labels. For each 
case study, we select the rules with the highest $\mathit{conf}$ and $\mathit{sup}$ from all the failure models we have generated for that case study. Table~\ref{tab:goal1} shows the input features that 

In this way, for each dataset, we can determine the input features that explain failure with the highest confidence and support. Our results are in Table~\ref{tab:goal1}.


%Each subset represents a combination of NTSS classes. So, in total, we develop $64$ features for autopilot and $255$ features for NTSS. 



%Recall from Section~\ref{sec:motivation} that the rules are meant to provide engineers with information on what combinations of the system input variables can explain failures with the highest confidence.  We first select features for learning failure models based on the inputs variables.  Both autopilot and NTSS case studies have eight inputs.  We consider all 64 subsets of the remaining six variables as features for learning failure models.  For NTSS, we consider the $255$ (i.e., $2^8-1$) subsets of the variables as input features. As discussed in Section~\ref{sec:motivation}, the purpose is to identify the bandwidth limits that the combination of NTSS classes  can take without compromising the network quality. Each subset represents a combination of NTSS classes. So, in total, we develop $64$ features for autopilot and $255$ features for NTSS. 

%in order to define features, we note two domain-specific considerations: (1)~ The reason is that the input variables of NTSS represent classes that already come with defined priority indices. Therefore, to identify the saturation limits of the combination of the adjacent classes, we consider the summation of their ordered subsets (i.e. 27 ) instead of all possible subsets (i.e. 255 subsets). 

%Hence, we consider the set of the following summations as features: $\{v_i+ v_{i+1}+\ldots+ v_{j}\}$ for $1 \leq i < j \leq 7$ where $v_i$ is an input variable. 


Next, we build failure models (both DT and DR) such that the input subsets are provided as the input features to the failure models (step 2). 
Recall from Section~\ref{subsec:fms} that both DR and DT generate a set of rules in the form \textsc{IF-condition-THEN-prediction}, where condition is a constraint over the input features and prediction is either pass or fail class. In our work, we consider the rules with fail as the prediction since we are interested in inferring rules characterizing failure conditions. Each rule comes with two metrics: confidence and support. Support ($\mathit{sup}$) shows the number of tests that satisfy the condition of the rule, and confidence ($\mathit{conf}$) shows what percentage of support has fail labels. For example, \textsc{IF Class6 + Class7 $>$ 300 THEN FAIL} has $\mathit{conf} = 100\%$ and $\mathit{sup} = 20$. This means that $20$ tests satisfy the condition of this rule, and all the $20$ tests have fail labels. Afterwards, we select the rules with the highest $\mathit{conf}$ and $\mathit{sup}$ for each case study (step 3). In this way, for each dataset, we can determine the input features that explain failure with the highest confidence and support. Our results are in Table~\ref{tab:goal1}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/RQ3process-sagacious.pdf}
    %\imagecaptionspace
    \caption{The process of inferring rules characterizing failure conditions obtained from our failure models.}\label{fig:RQ3Process}
\end{figure}

\emph{Results.} Table~\ref{tab:goal1} shows the input features and the number of times that their rules had the highest confidence and support among the datasets. As shown in the table, for the Autopilot case study, the rule that constrained $\mathit{ALT Mode}$, $\mathit{Turn Knob}$, $\mathit{Pitch Wheel}$ and $\mathit{Throttle}$ had the highest confidence and support in the majority of datasets for both DT and DR (i.e. 13/20 and 9/20 respectively). The confidence of this rule is $100\%$ and the support is on average $45$ for decision tree and $9$ for decision rules which are higher than those of the rest of the features. This rule suggests that due to the wide ranges of these four inputs, they are most likely to fail the requirement. Based on the autopilot handbook~\cite{??}, the values of these four inputs affect the attitude of airplane in reaching the desired altitude. Therefore, our findings help the engineers to test their systems for a more constrained and realistic environment reducing the number of spurious failures. For the NTSS case study, \textsc{IF Class5 + Class6 + Class7 > $89\%\cdot\mathit{totalbandwidth}$ THEN Fail} had the highest confidence and support in 9/10 datasets for DT (on average $\mathit{conf} = 100\%$ and $\mathit{sup} = 41$) and in all the datasets of DR (on average $\mathit{conf} = 93\%$ and $\mathit{sup} = 52$). Based on our investigation of the NTSS code, we realized that Class5, 6 and 7 are considered as the high priority classes under diffserv-8. Moreover, this rule indicates that less than $89\%$ of the total available bandwidth should be dedicated to the high-priority classes and engineers should carefully configure their NTSS so that a margin from the total bandwidth is assigned to the high-priority classes.

Further, for both case studies, on average DT generated more rules with $100\%$ confidence ($122$ for autopilot and $20$ for NTSS) compared to DR ($1.5$ for autopilot and $0.5$ for NTSS). This might be due to the process that DR follows to generate rules. In particular, DR first splits the data into two partitions: Grow and Prune. It starts by generating rules for the Grow set and prunes the rules using the Prune set. The rules are then added to a ruleset. The process continues until the length of the ruleset reaches a specific limit or there are no fail tests left in either of the Grow or Prune sets. However, there is no such  limitation for DT and the tree is expanded to the fullest extend resulting in more rules with $100\%$ confidence.

\input{Sections/goal1}

\begin{framed}
\noindent The answer to RQ3 is that the failure rules inferred by our FMs are in line with the public documentation available for our case studies.
\end{framed}


% \begingroup
% \begin{algorithm}[t]
% \parbox{0.95\columnwidth}{\caption{Surrogate-assisted test generation.}\label{alg:alg2}}

% \SetKwFunction{GenTests}{TestGeneration}
% \SetKwFunction{HandleImbalance}{HandleImbalance}
% \SetKwFunction{Simulate}{Simulate}
% \SetKwFunction{Train}{Train}
% \SetKwFunction{Predict}{Predict}
% \SetKwFunction{ChooseBestSurrogate}{ChooseBestSurrogate}
% \SetKwFunction{Reliability}{CheckReliability}
% \SetKwFunction{InitializeAndBalance}{InitializeAndBalance}
% \SetKwFunction{Execute}{Execute}

% \begin{algorithmic}[1]
% \INPUT- $S$: System
% \HINPUT- $\mathcal{R} = \{R_1, \ldots, R_n\}$: Ranges for input variables $v_1$ to $v_n$
% \HINPUT- $F$: Fitness function
% \HINPUT- $\textsc{Budget}$: Maximum number of fitness evaluations
% \OUTPUT- $\mathit{DS}$: A dataset to train failure models 

% %\STATE $\mathit{DS}^l$, $\mathit{DS}$ $\leftarrow$ \InitializeAndBalance {$S$, $\mathcal{R}$, $\mathcal{O}$}
% \STATE $\mathit{DS}\leftarrow $  \InitializeAndBalance {$S$, $\mathcal{R}$, $F$, $\frac{\textsc{Budget}}{2}$};
% \STATE $\mathit{DS}^l\leftarrow \mathit{DS}$; $\mathit{flag} \leftarrow $  $\top$; 
% %\COMMENT {The learn, analyze and test loop}
% \WHILE {$\frac{\textsc{Budget}}{2}$} 
%     \IF{($\mathit{flag}$)}
%     \STATE $(\mathit{SM}$, e) $\leftarrow$ \Train{$\mathit{DS}^l$}; \COMMENT {Training $\mathit{SM}$; $e$ is the error}
%      \ENDIF
    
%     \STATE $\mathit{t} \leftarrow$ \GenTests{$\mathcal{R}$, $1$}; %\COMMENT {Generate a test input}
%     \STATE $\bar{F}(t) \leftarrow $ $\mathit{SM}_{}.$ \Predict {$\mathit{t}$}; \COMMENT {Predict the fitness for $\mathit{t}$}
%    \IF{($\exists \sim \in \{\geq, <\}\cdot(\bar{F}(t) \sim 0) \wedge (\bar{F}(t) \pm e \sim 0)$}
%         \STATE $\mathit{DS} \leftarrow \mathit{DS} \cup \{\langle \mathit{t}, \bar{F}(t) \rangle \}$;  $\mathit{flag} \leftarrow \bot$; \COMMENT{Predicted fitness is used instead of the actual fitness}
        
%     \ELSE
%         \STATE \{$\langle t, F(t) \rangle\} \leftarrow $ \Execute{$S$,$\{t\}$, $F$}; \COMMENT{Compute fitness}
%         \STATE $\mathit{DS}^l \leftarrow \mathit{DS}^l \cup \{\langle \mathit{t}, F(t) \rangle \}$; $\mathit{DS} \leftarrow \mathit{DS} \cup \{\langle \mathit{t}, F(t) \rangle \}$; $\mathit{flag} \leftarrow \top$; \\
%     \ENDIF
    
% \ENDWHILE

% \RETURN $\mathit{DS}$
% \end{algorithmic}
% \end{algorithm}
% \endgroup


% \begingroup
% \begin{algorithm}[t]
% \parbox{0.95\columnwidth}{\caption{Preprocessing Phase (\textsc{InitializeAndBalance}).}\label{alg:alg1}}

% \SetKwFunction{GenTests}{TestGeneration}
% \SetKwFunction{HandleImbalance}{HandleImbalance}
% \SetKwFunction{Execute}{Execute}
% \SetKwFunction{TrainTune}{TrainAndTune}
% \SetKwFunction{Predict}{Predict}
% \SetKwFunction{ChooseBestSurrogate}{ChooseBestSurrogate}
% \SetKwFunction{Reliability}{CheckReliability}

% \begin{algorithmic}[1]
% \INPUT- $S$: System
% \HINPUT- $\mathcal{R} = \{R_1, \ldots, R_n\}$: Ranges for input variables $v_1$ to $v_n$
% \HINPUT- $F$: Fitness function  
% \HINPUT- $d$: The budgeted dataset size
% \OUTPUT- $\mathit{DS}$: A set of test inputs and their fitness values 

% %\COMMENT {Initial Testing. Generate $\frac{d}{2}$ test inputs}
% \STATE $\mathit{DS}^i$ $\leftarrow$ \GenTests {$\mathcal{R}$, $\frac{d}{2}$}; \COMMENT {(Adaptive) Random Testing}
% \STATE $\mathit{DS}^l \leftarrow$ \Execute{$S$, $\mathit{DS}^i$, $F$}; \COMMENT {Compute fitness values}
% %\COMMENT {Imbalance Handling. Generate $m$ test inputs using SMOTE to address imbalance datasets} 
% \STATE $\mathit{DS}^b$ $\leftarrow$ \HandleImbalance {$\mathit{DS}^l$};
% \STATE $\mathit{DS}^{b,l}$ $\leftarrow$ \Execute {$S$, $\mathit{DS}^b$, $F$}; \COMMENT {Compute fitness values}
% %\STATE $\mathit{DS}^i$ $\leftarrow$ \GenTests {$S$, $\mathcal{R}$, $\mathcal{O}$, $d - (m + n)$}; \COMMENT {Generate remaining tests using (Adaptive) Random Testing}
% \STATE  $DS$ $\leftarrow$ $\mathit{DS}^{b,l} \cup \mathit{DS}^l$;
% \RETURN $\mathit{DS}$
% \end{algorithmic}
% \end{algorithm}
% \endgroup

% \begingroup
% \begin{algorithm}[t]
% \parbox{0.95\columnwidth}{\caption{Dynamically Selecting Surrogates}\label{alg:alg3}}

% \SetKwFunction{GenTests}{TestGeneration}
% \SetKwFunction{HandleImbalance}{HandleImbalance}
% \SetKwFunction{Simulate}{Simulate}
% \SetKwFunction{Train}{Train}
% \SetKwFunction{Predict}{Predict}
% \SetKwFunction{ChooseBestSurrogate}{ChooseBestSurrogate}
% \SetKwFunction{Reliability}{CheckReliability}
% \vspace*{-.2cm}
% \hspace*{0.5cm}\ldots
% \begin{algorithmic}[1]
% \setalglineno{4}

%  \FOR {i = 0 to $\mathit{sm}$} 
% \STATE   ($\mathit{SM}_i$, $e_i$) $\leftarrow$ \Train {$\mathit{DS}^l$}; \COMMENT{Train several surrogate models}
% \ENDFOR
% \STATE $(\mathit{SM}, e) \leftarrow $ Select $\mathit{SM} \in \{\mathit{SM}_1, \ldots, \mathit{SM}_{\mathit{sm}}\}$ with the lowest error $e$

% \ldots     
% \end{algorithmic}
% \end{algorithm}
% \endgroup

% \begingroup
% \begin{algorithm}[t]
% \parbox{0.95\columnwidth}{\caption{ML-guided test generation (Regression Tree).}\label{alg:alg4}}

% \SetKwFunction{GenTests}{TestGeneration}
% \SetKwFunction{HandleImbalance}{HandleImbalance}
% \SetKwFunction{Simulate}{Simulate}
% \SetKwFunction{Train}{Train}
% \SetKwFunction{Predict}{Predict}
% \SetKwFunction{InitializeAndBalance}{InitializeAndBalance}
% \SetKwFunction{ExtractBoundaryRanges}{ExtractBoundaryRanges}
% \SetKwFunction{Execute}{Execute}

% \begin{algorithmic}[1]

% \INPUT- $S$: System
% \HINPUT- $\mathcal{R} = \{R_1, \ldots, R_n\}$: Ranges for input variables $v_1$ to $v_n$
% \HINPUT- $F$: Fitness function 
% \HINPUT- $\textsc{Budget}$: Maximum number of fitness evaluations
% %\HINPUT- $\mathit{th}$: Pass/Fail Threshold

% \OUTPUT- $\mathit{DS}$: A data set to train failure models 

% \STATE $\mathit{DS} \leftarrow $\InitializeAndBalance {$S$, $\mathcal{R}$, $F$, $\frac{\textsc{Budget}}{2}$};
% \WHILE {$\frac{\textsc{Budget}}{2}$}
%     \STATE $\mathit{RegTree}$ $\leftarrow$ \Train {$\mathit{DS}$};
%     \STATE $\{R'_{i_1}, \ldots, R'_{i_m}\} \leftarrow $ \ExtractBoundaryRanges {$\mathit{RegTree}$};
%     \FOR{$j \leftarrow 1$ to $m$ }
%       \STATE $\mathcal{R} \leftarrow (\mathcal{R} \setminus \{R_{i_j}\}) \cup \{R'_{i_j}\}$; \COMMENT {Replace ranges in $\mathcal{R}$ with those obtained from the regression tree}
%     \ENDFOR
%     \STATE $\{t\} \leftarrow$ \GenTests{$\mathcal{R}$, 1}; %\COMMENT {Generate a test in the reduced ranges}
%     \STATE $\mathit{DS}$ $\leftarrow$ $\mathit{DS}$ $\cup$ \Execute{$S$, $\{t\}$, $F$};\COMMENT {Compute fitness for $t$ and add to $\mathit{DS}$}
% \ENDWHILE
% \RETURN $\mathit{DS}$
% \end{algorithmic}
% \end{algorithm}
% \endgroup


% \begingroup
% \begin{algorithm}[t]
% \parbox{0.95\columnwidth}{\caption{ML-guided test generation (Logistic Regression).}\label{alg:alg5}}

% \SetKwFunction{GenTests}{TestGeneration}
% \SetKwFunction{HandleImbalance}{HandleImbalance}
% \SetKwFunction{Simulate}{Simulate}
% \SetKwFunction{Train}{Train}
% \SetKwFunction{Predict}{Predict}
% \SetKwFunction{InitializeAndBalance}{InitializeAndBalance}
% \SetKwFunction{GenerateCloseToRegBorder}{GenerateCloseToRegBorder}
% \SetKwFunction{Probability}{Probability}
% \SetKwFunction{Execute}{Execute}

% \begin{algorithmic}[1]

% \INPUT- $S$: System
% \HINPUT- $\mathcal{R} = \{R_1, \ldots, R_n\}$: Ranges for input variables $v_1$ to $v_n$
% \HINPUT- $F$: Fitness function
% \HINPUT- $\textsc{Budget}$: Maximum number of fitness evaluations

% \OUTPUT- $\mathit{DS}$: A data set to train failure models 

% \STATE $\mathit{DS} \leftarrow $ \InitializeAndBalance {$S$, $\mathcal{R}$, $F$, $\frac{\textsc{Budget}}{2}$};
% \WHILE {$\frac{\textsc{Budget}}{2}$}
%     \STATE $\mathit{LogReg}$ $\leftarrow$ \Train {$\mathit{DS}$};
%     \STATE $p \leftarrow $ \Probability {$\mathit{DS}$}; \COMMENT {probability of pass in $\mathit{DS}$}
%     \STATE $t$ $\leftarrow$ \GenerateCloseToRegBorder{$\mathcal{R}$, $\mathit{LogReg}$, $p$}; \COMMENT {select a test close to the regression border for $p$}
%     \STATE  $\mathit{DS}$ $\leftarrow$ $\mathit{DS}$ $\cup$ \Execute{$S$, $\mathit{\{t\}}$, $F$};%\COMMENT {Execute and add the test to the dataset}
% \ENDWHILE
% \RETURN $\mathit{DS}$
% \end{algorithmic}
% \end{algorithm}
% \endgroup


\begin{table*}[t]
\color{red}
\caption{Names, descriptions, the number of requirements and the identifiers of our study subjects. For each subject, we indicate  if it is computer-intensive (CI). All artifacts including requirements statements are available in our supplementary material~\cite{requirements}. }
\label{tab:simulinkmodels}
\vspace*{-.4cm}
\scalebox{0.48}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Description}}                                                    & \multicolumn{1}{c|}{\textbf{\#Reqs}} & {\textbf{ID}} & \multicolumn{1}{c|}{\textbf{CI}} \\ \hline
 Tustin                             & A common flight control utility for computing the Tustin Integration -- A Simulink model with                          57 blocks.                              & 9                                   &TU1$\ldots$TU9& \ding{55}                                                               \\ \hline
 Regulator                          & A regulators inner loop architecture used in many feedback control applications -- A Simulink model with 308  blocks.                                 &      1          & REG  &\ding{55}                                   \\ \hline
                                Nonlinear Guidance                 & A nonlinear algorithm for generating a guidance command for an air vehicle -- A Simulink model with                    373   blocks.                                 &   1                                 & NLG & \ding{55}  
\\ \hline
                                Finite State Machine                 & A finite state machine to enable
autopilot mode if a hazardous situation is identified -- A Simulink model with                       303   blocks.                                 &   1                                  & FSM & \ding{55}    
\\ \hline
                                 Autopilot                          & A single-engine, high-wing, propeller-driven aircraft simulation with all six degrees of freedom -- A Simulink model with  1549 blocks.                                 & 3                                     &  AP1, AP2, AP3 &  \ding{51}                                \\ \hline


 Network Traffic Shaping System & An NTSS testbed~\cite{enrich} developed using three virtual machines and based on OpenWRT~\cite{openwrt}. 

 & 1 & NTSS & \ding{51}  \\ \hline


\end{tabular}}
\vspace*{-.35cm}
\end{table*}

@article{enrich,
  title={Learning Non-robustness using Simulation-based Testing: a Network Traffic-shaping Case Study},
  author={Jodat, Baharin Aliashrafi and Nejati, Shiva and Sabetzadeh, Mehrdad and Saavedra, Patricio},
  journal={arXiv preprint arXiv:2212.08726},
  year={2022},
  pages={to appear in 16th IEEE International Conference on Software Testing, Verification and Validation (ICST 2023)}
}

==> Sections/todo.tex <==











==> headerpackages.tex <==
\usepackage{amsfonts}
\usepackage{ltl}

\usepackage{stmaryrd}
\usepackage{amsthm}
%\usepackage[utf8]{inputenc}
\usepackage{xcolor}
\usepackage[english]{babel} 
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{gensymb}
\usepackage{tikz}
\usepackage[inline]{enumitem}
\usepackage{numprint}
\usepackage{mathtools}
\usepackage[switch]{lineno}
\usepackage{gensymb}
\usepackage{amsmath}
\usepackage{fancybox}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage[xcolor=orange]{changes}
\usepackage{xcolor}
\usepackage[most]{tcolorbox}
\usepackage{fancybox}
\usepackage{pifont}% http://ctan.org/pkg/pifont

\newtcolorbox{mybox}[2][]{%  attach boxed title to top center
               %= {yshift=-8pt},
  colback      = gray!5!white,
  colframe     = gray!75!black,
  fonttitle    = \bfseries,
  colbacktitle = gray!85!black,
  left=0pt,
right=0pt,
top=0pt,
bottom=0pt,
%  title        = #2,#1,
 % enhanced,
}




\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}

%\newcommand\goal[1]{
%\noindent 
%\fcolorbox{black}{lightgray}{\noindent 
% \parbox{\columnwidth}{\noindent  #1}}\\
%}

\newcommand\objective[1]{
\vspace{0.1cm}
\noindent \fcolorbox{lightgray!40!black}{lightgray}{\parbox{0.98\columnwidth}{\noindent 
#1}}\vspace{0.1cm}\\
}


\definecolor{lightyellow}{rgb}{1.0, 1.0, 0.88}
\newcommand\defbox[1]{
\vspace{0.1cm}
\noindent \fcolorbox{lightyellow!40!black}{lightyellow}{\parbox{0.98\columnwidth}{\noindent 
#1}}\vspace{0.1cm}\\
}


\newcommand\resq[1]{
\noindent 
\fcolorbox{green!40!black}{green!5}{\noindent 
 \parbox{0.98\columnwidth}{\noindent  #1}}\\
}

\newcommand\hypothesis[1]{
\noindent 
\fcolorbox{yellow!40!black}{yellow!5}{\noindent 
 \parbox{0.98\columnwidth}{\noindent  #1}}\\
}


 \newcommand{\assumption}[2]{
\vspace{0.19cm} 
 \noindent \fcolorbox{black}{lightgray}{\parbox{0.98\columnwidth}{\noindent 
\textbf{\textsc{A#1.}} #2}}
\vspace{0.01cm}\\
} 
 
 
%  \newcommand{\assumption}[1]{\textbf{\textsc{A#1.}}} 




\definecolor{myBlue}{RGB}{0,133,255}%{HTML}{0085ff}
\definecolor{myGreen}{RGB}{0,115,0}

\newcommand\phase[1]{\tikz[baseline=(X.base)]\node [draw=myBlue,fill=myBlue,thick,rectangle,inner sep=2pt, rounded corners=2pt](X){\color{white}\textbf{#1}};}
\newcommand\phasenew[1]{\tikz[baseline=(X.base)]\node [draw=myGreen,fill=myGreen,thick,rectangle,inner sep=2pt, rounded corners=2pt](X){\color{white}\textbf{#1}};}


\newcommand\universeofInputs{\ensuremath{I}}
\newcommand\universeofOutputs{\ensuremath{O}}
\newcommand\universeofVariables{\ensuremath{V}}
\newcommand\interpretation[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand\specificationuniverse{S}
\newcommand\specification{s}
\newcommand\expectedoutputs{\ensuremath{E_o}}
\newcommand\timedomain{\ensuremath{\mathbb{T}}}
\newcommand\real{\ensuremath{\mathbb{R}}}
\newcommand\integer{\ensuremath{\mathbb{Z}}}
\newcommand\SFFOformula{\ensuremath{\varphi}}

\newcommand\formula{\ensuremath{\varphi}}
\newcommand\testcase{\ensuremath{\langle \timeinterval, \interpretation{\inputs}, \system \rangle}}


\newcommand\tollerableviolation{\ensuremath{\iota}}
\newcommand\noisevalues{\ensuremath{N}}
\newcommand\possibletestcase{\ensuremath{\langle \timedomain, \uncertainsystem,  \interpretation{\inputs}, \interpretation{\noises},   \interpretation{\parameters} \rangle}}



\newcommand\possibletestcaseprime{\ensuremath{\langle \timeinterval, \interpretation{\variables}, \interpretation{\inputsignals}, \noisevalues^\prime,  \system, \paramenters^\prime \rangle}}

\newcommand\partialsimulation{\ensuremath{F_o^\prime=H^\prime(t, \uncertainsystem,C, \interpretation{R},  \interpretation{F_i(n)}, N )}}

\newcommand\testoracle{\ensuremath{\system_\formula}}



\newcommand\uncertainsystem{\ensuremath{M_p}}



% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\definechangesauthor[name={Claudio Menghi},color=orange]{CM}
\definechangesauthor[name={Shiva Nejati},color=red]{SN}
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}

\newboolean{showcomments}
\setboolean{showcomments}{true} % toggle to show or hide comments
\ifthenelse{\boolean{showcomments}}
{\newcommand{\nb}[2]{
  \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize#1}
  {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
 }
 \newcommand{\version}{\emph{\scriptsize$-$working$-$}}
}
{\newcommand{\nb}[2]{}
 \newcommand{\version}{}
}

\newcommand\claudio[1]{\nb{Claudio}{#1}}
\newcommand\shiva[1]{\nb{Shiva}{#1}}


 \newcommand{\goal}[1]{\textbf{\textsc{O#1}}} 

 
 \newcommand{\addedCM}[1]{\added[id=CM]{#1}}
\newcommand{\deletedCM}[1]{\deleted[id=CM]{#1}}
\newcommand{\replacedCM}[2]{\replaced[id=CM]{#2}{#1}}

\usepackage{makecell}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\partner}{LuxSpace}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}



\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{def}}}{=}}
\newcommand\variables{\ensuremath{R}}
\newcommand\signals{\ensuremath{F}}
\newcommand\inputsignals{\ensuremath{I}}

\newcommand\block{\ensuremath{B}}

\newcommand\inputsi{\ensuremath{F_i}}

\newcommand\timeinterval{\ensuremath{T}}
\newcommand\inputs{\ensuremath{I}}
\newcommand\inputsignal{\ensuremath{i}}
\newcommand\inputsuniverse{I}
\newcommand\noises{\ensuremath{\Delta}}
\newcommand\noise{\ensuremath{\delta}}

\newcommand\outputs{\ensuremath{O}}
\newcommand\outputsignal{\ensuremath{o}}

\newcommand{\powerset}{\raisebox{.15\baselineskip}{\Large\ensuremath{\wp}}}

\newcommand\risk{\emph{risk}}
\newcommand\diff{\emph{diff}}
\newcommand\ourlogic{RFOL}
\newcommand\casestudy{\textsf{SatEx}}
\newcommand\casestudyorbittime{two and a half hours}
\newcommand\casestudysimulationtime{YYYY minutes}
\newcommand\signaltrace{\ensuremath{w}}
\newcommand\variabletrace{\ensuremath{v}}
\newcommand\model{\ensuremath{\signaltrace}}
\newcommand\system{M}
\newcommand\parameters{\ensuremath{\Pi}}
\newcommand\parameter{\ensuremath{\pi}}

\newcommand\ourtool{\textttt{Sagacious}}


\newcommand\autopilot{Autopilot}
\makeatletter
\def\old@comma{,}
\catcode`\,=13
\def,{%
  \ifmmode%
    \old@comma\discretionary{}{}{}%
  \else%
    \old@comma%
  \fi%
}
\makeatother

\newcommand\term{\ensuremath{\theta}}
\newcommand\restrictedsffo{\ensuremath{RSFO}}


%\newcommand{\phase}[1]{%
%  \tikz[baseline=(text.base)]
%    {\node [draw,rounded corners] (text) {#1};}%
%}




%%%% Evaluation results

\npthousandsep{\,}






%\newcommand{\phase}[1]{%
%  \tikz[baseline=(text.base)]
%    {\node [draw,rounded corners] (text) {#1};}%
%}


\newcommand\numcasestudy{11}

\newtheorem{remark}{Remark}


%%%% Evaluation results
\newcommand\requirementNumber{90}
\newcommand\averageTimeOracleGeneration{1}
\newcommand\averageBlocksOracleGeneration{1}
\newcommand\averageConnectionsOracleGeneration{1}
\newcommand\averageSimulinkOracleGeneration{1}
\newcommand\averageSizeFormula{1}
\newcommand\percentagetimesaving{1\%}

\newcommand\newtext[1]{\color{blue} #1 \color{black}  }

\usepackage{algorithm}

\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{multirow}

